Diffusion Models for Black-Box Optimization

The goal of offline black-box optimization (BBO) is to optimize an expensive black-box function using a fixed dataset of function evaluations. Prior works consider forward approaches that learn surrogates to the black-box function and inverse approaches that directly map function values to corresponding points in the input domain of the black-box function. These approaches are limited by the quality of the offline dataset and the difficulty in learning one-to-many mappings in high dimensions, respectively. We propose Denoising Diffusion Optimization Models (DDOM), a new inverse approach for offline black-box optimization based on diffusion models. Given an offline dataset, DDOM learns a conditional generative model over the domain of the black-box function conditioned on the function values. We investigate several design choices in DDOM, such as re-weighting the dataset to focus on high function values and the use of classifier-free guidance at test-time to enable generalization to function values that can even exceed the dataset maxima. Empirically, we conduct experiments on the Design-Bench benchmark and show that DDOM achieves results competitive with state-of-the-art baselines.

==> abstract.tex <==
  % The Abstract paragraph should be indented 0.25 inch (1.5 picas) on
  % both left and right-hand margins. Use 10~point type, with a vertical
  % spacing of 11~points. The \textbf{Abstract} heading must be centered,
  % bold, and in point size 12. Two line spaces precede the
  % Abstract. The Abstract must be limited to one paragraph.
 The goal of offline black-box optimization (BBO) is to optimize an expensive black-box function using a fixed dataset of function evaluations.
 Prior works consider \textit{forward} approaches that learn surrogates to the black-box function and \textit{inverse} approaches that directly map function values to corresponding points in the input domain of the black-box function.
 These approaches are limited by the quality of the offline dataset and the difficulty in learning one-to-many mappings in high dimensions, respectively. 
 We propose Denoising Diffusion Optimization Models (\name{}), a new inverse approach for offline black-box optimization based on diffusion models. 
 Given an offline dataset, \name{} learns a conditional generative model over the domain of the black-box function conditioned on the function values.
 We investigate several design choices in \name{}, such as reweighting the dataset to focus on high function values and  the use of classifier-free guidance at test-time to enable generalization  to function values that can even exceed the dataset maxima.
 Empirically, we conduct experiments on the Design-Bench benchmark~\citep{design-bench} and show that \name{} achieves results competitive with state-of-the-art baselines.

%  While forward approaches suffer from generalize to high function values, inverse approaches are harder to learn when inputs are 
 
%  We consider the offline setup, where we only have access to a fixed dataset for evaluation.
  
%   Black-box optimization (BBO) problems are ubiquitous in the modern world. Expensive evaluation of the underlying black-box function gives rise to an offline BBO setting, where we have access to a limited dataset of past function evaluations. At the test time, we are only allowed to make a few queries to the function. A natural approach to this problem would be to fit a forward model to the data and perform gradient ascent to find the maxima. However, such methods often suffer from poor generalization for out-of-distribution points \todo{cite COMs}. 
%   Another approach is to learn the inverse of the function and then use a high function value in order to obtain maxima. Since the inverse might not be unique, methods like MINs \todo{cite} use a conditional generative model to learn this one-to-many mapping. In our work, we show that score-based diffusion models when combined with classifier-free guidance and loss reweighting perform very well on offline BBO tasks.
  % Diffusion models \todo{cite} have recently shown excellent performance for generative modeling. In this paper, we use the diffusion model with classifier-free guidance and loss reweighing to solve the offline BBO problem and show improved performance on Design-Bench tasks \todo{ rephrase and cite the last line}.
